F-ViTA: Foundation Model Guided Visible to Thermal Translation

Thermal imaging is crucial for scene understanding, particularly in low-light and nighttime conditions. However, collecting large thermal datasets is costly and labor-intensive due to the specialized equipment required for infrared image capture. To address this challenge, researchers have explored visible-to-thermal image translation. Most existing methods rely on Generative Adversarial Networks (GANs) or Diffusion Models (DMs), treating the task as a style transfer problem. As a result, these approaches attempt to learn both the modality distribution shift and underlying physical principles from limited training data. In this paper, we propose F-ViTA, a novel approach that leverages the general world knowledge embedded in foundation models to guide the diffusion process for improved translation. Specifically, we condition an InstructPix2Pix Diffusion Model with zero-shot masks and labels from foundation models such as SAM and Grounded DINO. This allows the model to learn meaningful correlations between scene objects and their thermal signatures in infrared imagery. Extensive experiments on five public datasets demonstrate that F-ViTA outperforms state-of-the-art (SOTA) methods. Furthermore, our model generalizes well to out-of-distribution (OOD) scenarios and can generate Long-Wave Infrared (LWIR), Mid-Wave Infrared (MWIR), and Near-Infrared (NIR) translations from the same visible image. Code: https://github.com/JayParanjape/F-ViTA/tree/master.

==> ICCV2025-Author-Kit-Feb/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> ICCV2025-Author-Kit-Feb/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> ICCV2025-Author-Kit-Feb/sec/4_experiments_v-1.tex <==
\section{Experiments and Results}

\subsection{Datasets}
\noindent \textbf{Long-Wave Infrared (LWIR): }We use the FLIR-ADAS \cite{FLIRADASDataset} and KAIST \cite{kaist} datasets within this wavelength range. FLIR-ADAS has thermal images in the range of $7.5-13.5 \mu m$. However, there is a slight misalignment between the natural and thermal images.  Therefore, we use the aligned version of this dataset \cite{FLIRalign}, which includes 4,890 training and 126 testing visible-thermal pairs. The KAIST dataset also contains thermal images within the $7.5$–$13.5 \mu m$ range, representing road scenes, with 12,538 training pairs and 2,252 testing pairs.

\noindent \textbf{Mid-Wave Infrared (MWIR): }We use two datasets to conduct experiments within this range. The OSU dataset \cite{osu} contains images from both the MWIR as well as the LWIR domain. There are 4,862 training pairs and 3,683 testing pairs. The LiTiV dataset \cite{litiv} also consists of scenes involving roads and pedestrians. It contains a total of 4,564 training and 1,761 testing pairs.

\noindent \textbf{Near Infrared (NIR): } We use the NIRScene \cite{nirscene} dataset to represent this wavelength, which contains sceneries and landscapes. This dataset is split into 381 training pairs and 96 testing pairs.

\subsection{Implementation Details}We use the SwinT-OGC checkpoint for Grounding DINO, swin large checkpoint for RAM and vit-base model for SAM. We retain the default settings of the foundation models during training as well as testing. The training was done on a single NVIDIA RTX6000 GPU with a batch size of 1. The base learning rate was set to 5e-5.
% \begin{table}
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}
% {@{\extracolsep{4pt}}c c c c c c c c c@{}}
% \toprule
%  & \multicolumn{4}{c}{FLIR-ADAS \cite{FLIRADASDataset}} & \multicolumn{4}{c}{KAIST \cite{kaist}} \\
% \cline{2-5} \cline{6-9} \\
% Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
% \midrule
% Pix2Pix \cite{pix2pix2017} & 199.06 & 0.38 & 0.30 & 16.34 & 132.04 & 0.22 & 0.69 & 21.25\\
% ThermalGAN \cite{thermalgan} & 407.01 & 0.60 & 0.15 & 11.59 & 277.85 & 0.24 & 0.66 & 19.74\\
% InfraGAN \cite{infragan} & 140.01 & 0.50 & \textbf{0.41} & 16.95 & 222.96 & 0.159 & 0.76 & \underline{22.97}\\
% EGGAN-M \cite{eggan} & 139.11 & 0.43 & 0.29 & 10.32 & 79.45 & 0.37 & 0.48 & 10.65\\
% EGGAN-U \cite{eggan} & 140.92 & 0.55 & 0.37 & 14.3 & 76.27 & 0.27 & 0.63 & 17.07\\
% % Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
% PID \cite{PID} & \textbf{84.26} & \underline{0.36} & 0.40 & \underline{17.26} & \textbf{51.69} & \underline{0.14} & 0.79 & \textbf{23.6}\\
% F-ViTA (Ours) & \underline{133.30} & \textbf{0.23} & \textbf{0.73} & \textbf{18.73} & \underline{76.18} & \underline{0.21} & \textbf{0.88} & 18.96\\
% \bottomrule
% \end{tabular}}
% \caption{Results on LWIR datasets. Bold - best, underline - second best}
% % \vskip-8pt
% \label{tab:lwir_results}
% \end{center}
% \end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
Pix2Pix \cite{pix2pix2017} & 199.06 & 0.38 & 0.30 & 16.34 \\
ThermalGAN \cite{thermalgan} & 407.01 & 0.60 & 0.15 & 11.59\\
InfraGAN \cite{infragan} & 140.01 & 0.50 & \underline{0.41} & 16.95\\
EGGAN-M \cite{eggan} & 139.11 & 0.43 & 0.29 & 10.32\\
EGGAN-U \cite{eggan} & 140.92 & 0.55 & 0.37 & 14.3\\
% Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
PID \cite{PID} & \textbf{84.26} & \underline{0.36} & 0.40 & \underline{17.26}\\
F-ViTA (Ours) & \underline{133.30} & \textbf{0.23} & \textbf{0.73} & \textbf{18.73}\\
\bottomrule
\end{tabular}}
\caption{Results on FLIR-ADAS \cite{FLIRADASDataset} dataset. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:flir_results}
\end{center}
\end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
Pix2Pix \cite{pix2pix2017} & 132.04 & 0.22 & 0.69 & 21.25\\
ThermalGAN \cite{thermalgan} & 277.85 & 0.24 & 0.66 & 19.74\\
InfraGAN \cite{infragan} & 222.96 & 0.159 & 0.76 & \underline{22.97}\\
EGGAN-M \cite{eggan} & 79.45 & 0.37 & 0.48 & 10.65\\
EGGAN-U \cite{eggan} & 76.27 & 0.27 & 0.63 & 17.07\\
% Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
PID \cite{PID} & \textbf{51.69} & \textbf{0.14} & \underline{0.79} & \textbf{23.6}\\
F-ViTA (Ours) & \underline{76.18} & \underline{0.21} & \textbf{0.88} & 18.96\\
\bottomrule
\end{tabular}}
\caption{Results on KAIST dataset \cite{kaist}. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:kaist_results}
\end{center}
\end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
EGGAN-M \cite{eggan} & 542.51 & 0.47 & 0.55 & 12.95\\
EGGAN-U \cite{eggan} & 75.76 & 0.18 & \textbf{0.86} & \underline{20.46}\\
% Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
PID \cite{PID} & 85.58 & 0.25 & 0.58 & 14.1\\
F-ViTA (Ours) & \textbf{61.97} & \textbf{0.15} & \underline{0.78} & \textbf{20.92}\\
\bottomrule
\end{tabular}}
\caption{Results on the OSU dataset \cite{osu}. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:osu_results}
\end{center}
\end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
InfraGAN \cite{infragan} & 241.42 & 0.36 & 0.87 & 17.15\\
EGGAN-M \cite{eggan} & 238.41 & 0.35 & 0.93 & 12.81\\
EGGAN-U \cite{eggan} & \underline{152.09} & 0.23 & 0.95 & 18.45\\
% Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
PID \cite{PID} & 179.65 & \underline{0.20} & \underline{0.95} & \underline{19.22}\\
F-ViTA (Ours) & \textbf{118.52} & \textbf{0.16} & \textbf{0.96} & \textbf{27.55}\\
\bottomrule
\end{tabular}}
\caption{Results on the LiTiV2012 dataset \cite{litiv}. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:litiv_results}
\end{center}
\end{table}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
EGGAN-M \cite{eggan} & 126.2 & 0.18 & 0.83 & 15.25\\
EGGAN-U \cite{eggan} & 125.6 & 0.23 & 0.79 & 18.45\\
% Instruct-Pix2Pix \cite{instructpix2pix} & 138.39 & 0.23 & 0.72 & 18.25 \\
PID \cite{PID} & 166.67 & 0.31 & 0.62 & 14.21\\
F-ViTA (Ours) & \textbf{63.67} & \textbf{0.11} & \textbf{0.85} & \textbf{19.23}\\
\bottomrule
\end{tabular}}
\caption{Results on the NIRScene dataset \cite{nirscene}. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:nirscene_results}
\end{center}
\end{table}

\subsection{Image Translation Experiments}
We compare our method with existing SOTA visible-to-thermal translators on five datasets. The results on FLIR-ADAS are tabulated in \cref{tab:flir_results}. We find that our method is able to outperform existing methods on multiple metrics, with a significant rise observed in SSIM. However, we see a lower FID score than the current SOTA. While FID compares the distributions between the ground truth and the generated thermal image, SSIM measures the structural and visual soundness of the generated image. Hence, both are important to gauge the quality of generation. On the KAIST dataset, as can be seen in \cref{tab:kaist_results}, we see a similar trend where the SSIM for our method is better but other metrics are comparable to PID. This is not surprising, given that PID models the physical quantities behind LWIR images and constrains the model accordingly. In contrast, our model captures the structure of objects better due to localization information present through the masks (causing improved SSIM), but at the same time has a slight tendency to miss the differences in output intensities for different parts of the same object (causing increased FID). This can happen since there are multiple similar signals from the prompts for different parts of the same object. In addition, note that FLIR is a comparatively smaller dataset than KAIST, which is why we see an overall better performance with our method.

\cref{tab:osu_results} shows the results on the OSU dataset, where we see a significant improvement in all metrics, while SSIM is comparable. Similarly, for LiTiV, as shown in \cref{tab:litiv_results}, and for NIRScene, as seen in \cref{tab:nirscene_results}, we find that our method outperforms all other methods across all metrics.  Note that these are cases of low-data regimes, where the advantages of our model are clearly demonstrated. We present qualitative results in \cref{fig:qual} across all five datasets used for comparison, selecting examples from both indoor and outdoor scenes. As shown in the figure, our method (third column) performs consistently well across all datasets. PID excels in LWIR but struggles to generate accurate translations for MWIR and shows an overall increased intensity in the NIR case. This is expected, as the theoretical analysis and formulation of PID are primarily designed for LWIR translations. In contrast, EGGAN-M and EGGAN-U slightly distort object structures, as observed in the figure. In comparison, our method, F-ViTA, generates thermal images that closely resemble the ground truth.

\begin{figure*}
  \centering
  {\includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/resources/qualitative.png}}
 \vskip-8pt 
 \caption{Qualitative Results over datasets from three different wavelength spectra. Our method (third column) is able to generate images more similar to the ground truth as compared to existing methods (fourth, fifth and sixth columns)s}  \label{fig:qual}
\end{figure*}

\subsection{Out-of-Distribution (OOD) Experiments}
%We use the MFNet \cite{mfnet} dataset for evaluating the generalizability of our method on the OOD data. MFNet contains visible images and their thermal counterparts in the LWIR range. As shown in \cref{tab:mfnet_ood_results}, F-ViTA, trained on the KAIST dataset is able to perform well on MFNet as compared to PID trained on KAIST. Similarly, for models tuned using only FLIR, our method performs significantly better than PID trained on the same dataset. PID first learns estimates for physical quantities related to the thermal dataset as a whole, while our method learns object-wise estimates implicitly. Hence, when transferred to a new dataset, our approach shows more robustness, which can be seen through the table. In addition, we also include one more experiment where we train F-ViTA using one dataset from each modality (KAIST for LWIR, LiTiV for MWIR and NIRScene or NIR) and then test its performance on MFNet with the instruction of converting it to a long wave infrared. We observe that even after the addition of additional modalities, the performance on MFNet remains comparable to when trained using just the LWIR KAIST dataset.

We use the MFNet \cite{mfnet} dataset to evaluate the generalizability of our method on out-of-distribution (OOD) data. MFNet contains visible images and their thermal counterparts in the LWIR range. As shown in \cref{tab:mfnet_ood_results}, F-ViTA, trained on the KAIST dataset, performs significantly better on MFNet compared to PID trained on KAIST. Similarly, for models tuned using only the FLIR dataset, our method outperforms PID trained on the same data. PID first learns estimates for physical quantities related to the thermal dataset as a whole, while our method implicitly learns object-wise estimates. As a result, our approach exhibits greater robustness when transferred to a new dataset, as reflected in the table. Additionally, we conduct an experiment where we train F-ViTA using one dataset from each modality (KAIST for LWIR, LiTiV for MWIR, and NIRScene or NIR for NIR) and then test its performance on MFNet with the instruction to convert to long-wave infrared. We find that even with the inclusion of additional modalities, the performance on MFNet remains comparable to when trained using only the LWIR KAIST dataset.

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c@{}}
\toprule
Method & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
PID \cite{PID} (tuned on KAIST) & 196.10 & 0.39 & 0.85 & 13.53\\
Ours (tuned on KAIST) & \textbf{70.98} & \textbf{0.30} & \textbf{0.87} & \textbf{16.33}\\
\midrule
PID \cite{PID} (tuned on FLIR-ADAS) & 142.60 & 0.47 & 0.70 & 12.02\\
Ours (tuned on FLIR-ADAS) & \textbf{100.54} & \textbf{0.35} & \textbf{0.81} & \textbf{12.85}\\
\midrule
Ours (tuned on all datasets from all wavelengths) & 94.5 & 0.37 & 0.83 & 13.72\\
\bottomrule
\end{tabular}}
\caption{OOD Results on the MFNet dataset \cite{mfnet}. Bold - best, underline - second best}
% \vskip-8pt
\label{tab:mfnet_ood_results}
\end{center}
\end{table}

\subsection{Text-Prompted Translation Experiments}
F-ViTA uses text instructions for guiding the diffusion model to perform the image translation. Hence, it is possible for it to learn to generate images for specific infrared spectra by specifying it in the instructions. To explore this, we train F-ViTA on KAIST (LWIR), OSU (MWIR), LiTiV (MWIR) and NIRSCENE (NIR) together with the type of image in the instruction. For instance, for KAIST, we ask the DM to generate a long wave infrared image. Once trained, we test the model's ability to generate all three types of IR images from a given RGB image from the test data. Some examples of such translations can be seen in \cref{fig:allmodal_translations}.
From the figure, we observe that F-ViTA produces reasonable predictions for LWIR, MWIR, and NIR given a single RGB image. The GT column represents the ground truth thermal image from the dataset-specific wavelength range. The first five rows display images from the test sets of the datasets on which the model was trained. The last three rows show predictions on MFNet, which was not used during training, demonstrating strong out-of-distribution (OOD) performance with F-ViTA. The final row illustrates a failure case where the model misses pedestrians in the MWIR and NIR predictions, indicating potential areas for improvement. Notably, no existing methods demonstrate such multi-spectral translation capability. We are the first to explore this direction with F-ViTA and encourage further research in this area.


\begin{figure*}
  \centering
  {\includegraphics[width=0.95\linewidth]{ICCV2025-Author-Kit-Feb/resources/allmodal_translations_300x.png}}
 \vskip-8pt 
 \caption{Text prompted translation capability of F-ViTA. Our method is able to generate LWIR, MWIR or NIR images based on the text instruction. The second column shows the ground truth which is from the wavelength range specified next to the dataset name on the right.}  \label{fig:allmodal_translations}
\end{figure*}

\subsection{Downstream Applications}

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c@{}}
\toprule
$\%$ original data used & MIoU (\(\uparrow\)) & Mean Pixel Accuracy (\(\uparrow\)) \\
\midrule
0 & 0.501 & 55.58\\
10 & 0.503 & 56.01\\
25 & 0.520 & 59.22\\
50 & 0.526 & 59.1\\
100 & 0.527 & 59.6\\
\bottomrule
\end{tabular}}
\caption{Results on MFNet \cite{mfnet} using Sigma \cite{sigma} as the RGB-T segmentation pipeline. The rows indicate the percentage of real thermal data used in the training data, with the rest of the data being synthetic. We see only a small drop in the metrics as we go up the table (more synthetic data used), towards the applicability of our method.}
% \vskip-8pt
\label{tab:rgbt_results}
\end{center}
\end{table}

\noindent \textbf{RGB-T Fusion for Segmentation: } Thermal imagery is often used for multi-modal segmentation, where the RGB image and its paired thermal image are processed and fused to produce the output segmentation map. We conduct experiments to show an application of our pipeline for thermal image generation. We use the F-VITA model, tuned on the KAIST dataset, to generate thermal images for the MFNet \cite{mfnet} dataset. Next, we generate five types of data for training a RGB-T segmentation model, using $0\%$, $10\%$, $25\%$, $50\%$, and $100\%$ of the actual thermal images respectively. The rest of the images are taken from the generated predictions from our model. We use the original thermal images for the testing data. We use the SOTA RGB-T fusion model, called Sigma \cite{sigma} for the segmentation task. Sigma uses the recently introduced V-Mamba framework along with a concatenation and cross-attention mechansim to effectively fuse the two modalities. With this setup, we train Sigma with the five datasets and test its performance, as tabulated in \cref{tab:rgbt_results}.

\noindent We observe that when only the original thermal data is used, Sigma gives a MIoU of $52.7$ and mean pixel accuracy of $59.6$. When we replace $50\%$ of the data with the synthetic data generated with our method, the MIoU drops to $52.6$ and accuracy to $59.1$, which is not a significant drop compared to the reduction in original training data. With an all-synthetic training set, these numbers only reduce by 4 points. Note that the thermal data was created using F-ViTA trained on KAIST only, thus being OOD for the generation model. Thus, these results also denote the quality of our predictions.

\begin{table}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c@{}}
\toprule
$\%$ original data used & MIoU (\(\uparrow\)) & Mean Pixel Accuracy (\(\uparrow\)) \\
\midrule
0 & 0.30 & 43.38\\
10 & 0.30 & 45.24\\
25 & 0.30 & 40.01\\
50 & 0.38 & 51.29\\
100 & 0.38 & 54.12\\
\bottomrule
\end{tabular}}
\caption{Results on MFNet \cite{mfnet} using Segformer \cite{segformer} for thermal segmentation for 10 classes. The rows indicate the percentage of real thermal data used in the training data, with the rest of the data being synthetic. We see a slight drop in the metrics as we go up the table (more synthetic data used), which suggests a use case of F-ViTA for synthetic data generation.}
% \vskip-8pt
\label{tab:thermal_results}
\end{center}
\end{table}

\noindent \textbf{Thermal Image Segmentation: }In this experiment, we train a Segformer \cite{segformer} on the thermal training data using the same mixtures as in the previous experiment, and then evaluate its performance on the test data containing original thermal images. Note that we do not use RGB images here, making this a purely semantic segmentation task based on thermal images. As shown in \cref{tab:thermal_results}, with 100\% original training data, we achieve a MIoU of 0.38 and a mean accuracy of 54\%. Even when replacing 50\% of the data with synthetic images, we observe comparable performance. Below this threshold, we see a noticeable decrease in accuracy, suggesting areas for further exploration. Nevertheless, the predictions from our method offer a viable alternative to capturing infrared images using specialized hardware.


\subsection{Ablation Studies}
We perform an ablation study over the components extracted from the foundation models that are passed to the diffusion process. As seen in \cref{tab:ablation_components}, when neither of text, bounding boxes or mask embeddings are used (first row), we see a lower performance in all metrics. Adding just the text tags identified from the image (second row) improves these metrics. The text tags are extracted using the RAM model, and converted into embeddings using CLIP before passing to the DM. Next, we add only the embeddings from the bounding boxes for the objects detected by Grounding DINO (third row) and see on par metric values. However, adding msk embeddings from Grounded SAM (fourth row) gives us a slight improvement. This is expected since masks provide more precise localization than bounding boxes. In addition, unlike masks, a  bounding box around bigger objects like buildings or trees may also encompass other objects like vehicles or people. Hence, we see an advantage when using masks. In the fifth row, we use both the text tags and the bounding boxes, which slightly improves the performance over second and third rows, where they are passed separately. Finally, the last row denotes the case used in F-ViTA, with both the text embeddings and mask embeddings being provided to the DM. We see that this case improves over all other rows, since text and masks provide the localization and semantic information about the objects to the DM. We do not include cases where box and mask embeddings are used, since adding boxes is superfluous in the presence of masks.
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}
{@{\extracolsep{4pt}}c c c c c c c@{}}
\toprule
Text Labels & Bounding Boxes & Masks & FID (\(\downarrow\)) & LPIPS (\(\downarrow\)) & SSIM (\(\uparrow\)) & PSNR (\(\uparrow\)) \\
\midrule
& & & 80.03& 0.18 & 0.72 & 19.64\\
\checkmark & & & 76.43 & 0.20 & 0.74 & 20.5\\
 & \checkmark & & 76.01 & 0.20 & 0.75 & 20.01\\
& & \checkmark & 69.81 & 0.19 & 0.76 & 20.7\\
\checkmark & \checkmark & & 75.18 & 0.17 & 0.76 & 20.24\\
\checkmark & & \checkmark & \textbf{61.97} & \textbf{0.15} & \textbf{0.78} & \textbf{20.92}\\
\bottomrule
\end{tabular}}
\caption{Ablation over the components passed to the diffusion process using the FM. \checkmark indicates the component being used, with the first row indicating neither text, boxes or masks being used and the last row indicating F-ViTA where text and masks are used.}
% \vskip-8pt
\label{tab:ablation_components}
\end{center}
\end{table}
